Introducing the structural bases of typicality effects in deep learning

In this paper, we hypothesize that the effects of the degree of typicality in natural semantic categories can be generated based on the structure of artificial categories learned with deep learning models. Motivated by the human approach to representing natural semantic categories and based on the Prototype Theory foundations, we propose a novel Computational Prototype Model (CPM) to represent the internal structure of semantic categories. Unlike other prototype learning approaches, our mathematical framework proposes a first approach to provide deep neural networks with the ability to model abstract semantic concepts such as category central semantic meaning, typicality degree of an object's image, and family resemblance relationship. We proposed several methodologies based on the typicality's concept to evaluate our CPM-model in image semantic processing tasks such as image classification, a global semantic description, and transfer learning. Our experiments on different image datasets, such as ImageNet and Coco, showed that our approach might be an admissible proposition in the effort to endow machines with greater power of abstraction for the semantic representation of objects' categories.

==> tex/1_introduction_old.tex <==
% !TeX spellcheck = en_US
\section{Introduction}
\label{sec:introduction}
% \IEEEPARstart{M}{emory}
 Memory is one of the most amazing faculties of the human being and construed as the brain's ability to code, store, and retrieve information~\cite{atkinson1968}. Semantic memory~\cite{tulving2007coding}, for instance, refers to general world knowledge that we accumulate throughout our lives~\cite{mcrae2013}. A relevant aspect of the functional neuroanatomy of the semantic memory resides in the representation of the meaning  and the  properties~\cite{martin2007representation} of objects. Several observations indicate that human beings are capable of: \textit{i)}~learning the most distinctive features of a specific object category~\cite{martin2007representation,thompson2003neuroimaging} and \textit{ ii)}~producing categories and~object semantic definitions~(abstractions) at a very early age~\cite{martin2007representation}. Since, semantic memory involves the semantic definition of objects~\cite{tulving2007coding}, the success of object recognition, classification, and description tasks is strongly related to the success of recovering the learned knowledge~\cite{tulving2007coding}.
 
For several years, the fields of Image Processing and Computer Vision have developed pattern recognition methods with an impressive performance some specific tasks, but still lacking in others when compared to human proficiency. Although state-of-the-art methods have achieved remarkable results, there are still many challenges to attain the discriminative power and the abstraction of semantic memory to represent the semantic of visually acquired information. How to infer or ascribe semantics to objects? How to emulate the behavior of semantic memory in the representation of learned knowledge of objects' features? How to extract and encode such features to encapsulate the representation of the meaning (or semantic representation) of a specific object? How to learn the definition of semantic categories and use this definition in object recognition, classification, and description tasks? The quest to answer some of these questions still occupy the investigation agenda of many researchers.

\begin{figure*}[t]
	\begin{center}
		
		%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
		\includegraphics[width=0.88\linewidth]{figs/Fig1MotivationConcepts.pdf}% egfigure.eps
	\end{center}
	 \vspace*{-\baselineskip}
	\caption{\textbf{Motivation and Concepts}. Schematic of our prototype-based description model. The human visual system is able to observe and build the semantic description of an object based on its  most distinctive features within that object's category. We propose a prototype-based model to simulate this behavior through the pipeline  composed of  modules \textit{1)} to \textit{6)}.
		\textit{1)} features extraction; \textit{2)} recognition of object features; \textit{3)} categorization based on prototypes; \textit{4)} object features; \textit{5)} central semantic meaning of a  category~(the category prototype); \textit{6)} our Global Semantic Description based on Prototypes.}
	\label{fig:motivation}
	
\end{figure*}


In this paper\footnote{This paper is an extension of the published conference paper~\cite{vidal2019WACV}.} -- motivated by the semantic memory behavior -- we propose a mathematical framework that endeavors to represent the semantic definition of object categories. We also propose a procedure to introduce this semantic representation of object categories in the global semantic description and classification of objects features extracted from images.

Image semantic understanding is influenced by how the features of image basic components~(\eg, objects) are semantically represented, and the semantic relations between these basic components~\cite{guo2016deep}. Current models for knowledge extraction (high-level vision processes) from images are highly influenced by the methods used to detect, extract, and represent image relevant semantic information. 
%Consequently, the extraction of image features has been the subject of Computer Vision research for decades.

For several years, hand-crafted features~\cite{bay2008SURF,lowe2004SIFT,tola2008DAISY} and machine learning methods~\cite{simonyan2014learning,strecha2012ldahash} have been the choice for image feature description tasks.
The advent of Convolutional Neural Networks~(CNN) outperformed those traditional methods used for image feature representation, %n~\cite{bay2008SURF,lowe2004SIFT,tola2008DAISY} %\cite{bay2008SURF,lowe2004SIFT,tola2008DAISY,simonyan2014learning,strecha2012ldahash}
% and enabled to achieve a visual recognition model with similar behavior of \textit{human semantic memory}~\cite{tulving2007coding} for classification tasks \cite{he2016deep,simonyan2014very,szegedy2017inception}, sparking the tendency of images semantic processing with deep-learning techniques. Representations of image features extracted using deep classification models \cite{he2016deep,simonyan2014very,szegedy2017inception}, or using  CNN-descriptors are commonly referred to as \textit{semantic feature} or \textit{semantic signature}. %zbontar2015computing
%The Convolutional Neural Networks~(CNN) success
and spawned numerous CNN-descriptors produced with different approaches that learn effective representations for describing image features \cite{kim2017fcss,simo2015discriminative,zagoruyko2015learning}. 
Consequently, representations of image features extracted using deep classification models \cite{he2016deep,simonyan2014very,szegedy2017inception}, or using  CNN-descriptors are commonly referred as semantic feature or semantic signature. Nevertheless, none of these models codify the representation of the visual information based on the theoretical foundation of Cognitive Science to represent the semantic meaning.
%han2015matchnet


%
%In this paper -- motivated by the semantic memory behavior -- we propose a mathematical framework that attempts to represent the semantic definition of object categories. Also, we propose a procedure to introduce this semantic representation of object categories in the global description of objects features extracted from images.



%This human learning capacity is so perfect and robust that, for example, when presented with an image, a glance is sufficient for a human to point out and describe minute details present therein~\cite{fei2007we,karpathy2015deep}. However, what are the semantic features that are actually extracted so efficiently? How are these represented in the human brain? Moreover, how is learning accomplished based on the sensory of the visual system and its connections? These are just some of the intriguing questions that have occupied the investigation agenda of many research areas.

%\IEEEPARstart{T}{he}

%The advent of Convolutional Neural Networks~(CNN) outperformed handcrafted feature extraction and enabled us to achieve a visual recognition model with similar behavior of \textit{semantic memory} for classification tasks \cite{he2016deep,simonyan2014very,szegedy2017inception}, sparking the tendency of images semantic processing with deep-learning techniques. 

%rosch1988coherences

\textit{Semantic feature} and \textit{Semantic Meaning} terms have been extensively studied in the field of linguistic semantic. While, according to Fromkin~\etal ~\cite{fromkin2018introduction}, a semantic feature is defined as the representation of the basic conceptual components of the meaning of any lexical item, Rosch~\cite{rosch1975cognitive} holds that the representation of semantic meaning is related to the category prototype, particularly to those categories denoting natural objects. In her seminal work~\cite{rosch1975cognitive}, Rosch introduced the concept of semantic prototype and presented an in-depth analysis of the semantic structure of the meaning of words. The Prototype Theory~\cite{rosch1975cognitive,rosch1975family,rosch1978principles,rosch1978cognition} proposes that human beings think of categories in terms of abstract prototypes, represented by typical members of the category. This theory also indicates that successful execution of object recognition and description tasks in the human brain is inherently related to the learned prototype of the object category~\cite{rosch1975cognitive,rosch1978principles,minda2002comparing,zaki2003prototype}. 
%
%The term \textit{Semantic feature} has been extensively studied in the field of linguistic semantic; it is defined as the representation of the basic conceptual components of the meaning of any lexical item \cite{fromkin2018introduction}. 
%
%Image semantic understanding is influenced by how are semantically represented the features of image basic components~(\eg, objects), and the semantic relations between these basic components~\cite{guo2016deep}. CNN-description models \cite{han2015matchnet,lin2016learning,simo2015discriminative,zagoruyko2015learning} and semantic description models~\cite{han2017scnet,kim2017fcss,Rocco18} stand for the semantic information of image features using a range of different approaches.  
%
%CNN description models do not codify their representation based on the Cognitive Science foundations to represent the meaning zbontar2015computing, choy2016universal
%
In this paper, we rely on cognitive semantic studies related to the Prototype Theory for modeling the central semantic meaning of objects categories: the prototype.
We propose a novel approach to take on the semantic features descriptions of objects based on prototypes. Our \textit{prototype-based description model} uses the category's prototype to find a global semantic representation of the basics conceptual components (objects) of the image meaning. Also, we propose a \textit{prototype-based semantic classification model} that uses prototypes as neuron prior knowledge to classify object's image based on its semantic distinctiveness.

We apply the Prototype Theory as a theoretical foundation to represent the semantic meaning of the visual information lying in the basics components of a scene: objects. 
The observations on the Prototype Theory raise the following two questions: i) Can a model of the perception system be developed in which objects are described using the same semantic features that are learned to identify and classify them? ii) How can the category prototype be included in the object global semantic description and classification tasks?
%



% In this paper, we rely on cognitive semantics studies related to the Prototype Theory for modeling the \textit{central semantic meaning} of object categories. Our approach uses the representation of \textit{central semantic meaning} of category for simulating the human behavior in object features description task.


%Human beings can learn the most distinctive features of a specific category~\cite{martin2007representation,thompson2003neuroimaging}. These learned features (or properties) are used by the human brain to identify, classify, and describe objects~\cite{tulving2007coding}.


We address these two questions motivated by the human's approach to classifying and describing objects globally. Humans use the generalization and discrimination processes to build object descriptions that highlighting their most distinctive features within the category. 
For example, a typical human description: a dalmatian is a dog~(generalization ability to recognize the central semantic meaning of dog category) distinguished by its unique black or liver-colored spotted coat~(discrimination ability to detect the semantic distinctiveness of object within the dog category). Figure~\ref{fig:motivation} illustrates the intuition and concepts of our prototype-based description model.

Our experiments show that our mathematical framework~(semantic prototype and semantic distance metric) allows us to interpret possible semantic associations between members within the category's internal structure. Results show that a relationship could be established between the proposed semantic distance metric and the representativeness of the object's image. Our image global semantic descriptor's performance evaluation shows that it can outperform other types of global representations of images for some computer vision tasks.  The image signature also encapsulates the object's semantic information (object's semantic value and typicality score). Furthermore, the experiments show that the CNN-Layer architecture of our  prototype-based classification model can achieve good performance while conferring the higher interpretation power of the CNN models. This was made possible due to the simplicity and more explicit geometric interpretation of the mathematical framework we developed for categories.

%Our experiments showed that our image global semantic representation based on category prototypes could outperform other image global representations in some computer vision tasks. Also,  note that our GSDP encoding can describe objects images while encapsulates in its image signature the object's semantic information (object semantic value and object typicality score).
%Experiments showed that lowest dimensional GSDP representations (for each CNN model) were the ones that achieved the best size-performance trade-off.

%The results achieved in clustering tasks encourage us to evaluate the generalization ability of our semantic representation in other computer vision tasks as image retrieval

% More specifically,
 The main contributions of this work are as follows:
\begin{enumerate}
	\item a \textit{Computational Prototype Model}~(CPM). A  mathematical framework based on the foundations of Prototype Theory to represent the central semantic meaning of the images of object categories. % Our CPM model allows to interpret  possible semantic associations between members  within the category internal structure.
	
	\item a \textit{semantic distance metric} in object image CNN features domain, which can be construed as a measure of object typicality within the object's category. %Our experiments show that a relationship can be established between the semantic distance metric proposed and object image visual representativeness.
	\item a \textit{prototype-based description model} for global semantic description of object's images. Our semantic description model introduces, for the first time, the use of category prototypes in image global description task.
	\item a \textit{prototype-based semantic classification model}  for semantic classification  of object's images. We propose a CNN-Layer architecture that classifies objects according to its similarity to our prototype encoding.
\end{enumerate}


%For example, a typical human description: a dalmatian is a dog~(central semantic meaning) that is distinguished by its unique black or liver-colored spotted coat~(semantic difference concerning the central semantic meaning of dog category). Figure~\ref{fig:motivation} depicts our prototype-based description model.

%We evaluate our approach using CNN-models both on MNIST and ImageNet datasets. The experiments show that our prototype-based description model can simulate the prototypical organization of objects categories. Furthermore, our descriptor can construct semantic signatures that are discriminative, interpretable, with low dimensionality, and with the ability to encapsulate and to retain the meaning of object features.

%\todo{Add a paragraph here describing briefly the results}.



%The main idea is to use the quality of the features extracted by classification models both to represent the central semantic meaning of a specific category, and also to learn to represent its specificities within the category.



==> tex/5_conclusions_old.tex <==
\section{Conclusion}

%Motivated by how human beings represent and relate the meanings attributed to objects, this research was based on the Prototype Theory to propose semantic representations of object categories and object images. 
This paper introduced and evaluated three models based on the foundations of Prototype Theory: a Computational Prototype Model~(CPM), a novel Prototype-based Description Model~(GSDP), and a Prototype-based Classification Model. While the CPM model provides a representation of the internal semantic structure of object categories, the GSDP descriptor uses the CPM components (semantic prototype and semantic distance metric) to extract a semantic representation of objects. The prototype-based classification model uses CPM constraints to learn object categories.

Our experiments showed that the CPM model could encapsulate relevant features of the object's category in our semantic prototype representation. Moreover, we showed that the semantic distance metric proposed in this paper could simulate semantic relationships in terms of visual typicality between category members. Our prototypical distance can be understood as an object's image typicality score. The CPM model can capture the object's visual typicality and the central and peripheral meaning of objects' categories. 

%We proposed the CPM model to represent the internal semantic structure of object categories. Experiments showed that our CPM model was able to encapsulate relevant features of objects category in our semantic prototype representation. Also, we showed that our semantic distance metric could simulate semantic relationships in terms of visual typicality, between category members. %Our experiments showed that a relationship could be established between our semantic distance metric and object image visual representativeness.
%Expressly, our prototypical distance can be understood as an object image typicality score. That is, our CPM model can capture the object's visual typicality and the central and peripheral meaning of objects categories. 


%We proposed a prototype-based description model that uses the CPM model main components (\textit{semantic prototype} + \textit{semantic distance metric}) to construct a semantic representation of  object's image. 

Our prototype-based description built a discriminatory signature that semantically describes objects' images highlighting its most distinctive features within the category. The GSDP descriptor\footnote{All source code, prototypes datasets, and GSDP tool tutorials are publicly available in our lab's Github: https://github.com/verlab/gsdp.} introduces a new approach to the semantic description of objects' images. GSDP descriptor does not need to be trained, and it is scalable and easily adaptable to be used with any CNN classification model. Experiments in large image datasets show that our global semantic descriptor is discriminative, small dimensioned, and encodes the semantic information of category members. We further showed that our GSDP object representation preserves the object's semantic meaning and the object typicality score in its taxonomy.   

%Our novel GSDP\footnote{All source code, prototypes datasets, and tutorials are publicly available in our lab's Github: https://github.com/verlab/gsdp.} representation introduces a new approach to the semantic description of object images; and experiments in large image dataset shows that is discriminative, small dimensioned, and encodes the semantic information of category members. %We propose to replace the softmax layer of common CNN models for our PS-Layer to use the image typicality property to learn object categories. 

Furthermore, we present a prototype-based classification model that uses the CPM model constraints to learning object categories. Our PS-Layer introduces the image typicality property in the semantic category learning process, and experiments conducted showed that it could outperform some CNN-Models architectures. Our PS-Layer also provides higher interpretive power to CNN models due to simplicity and clear geometric interpretation of the object typicality concept.



\subsection*{Limitations and Future works}
The proposed prototype-based description model was constructed strictly to describe objects' images, not to describe scenes' images. Moreover, we did not evaluate our CPM model in a dataset with annotations of the image typicality. Consequently, as future work, we intend to construct a new image dataset with typicality annotations according to the interpretation criteria of human beings.
%Note that even when our semantic descriptor was evaluated in images that representing scenes, our GSDP descriptor can outperform other image global representations. 
Regarding the prototype-based classification method, it requires prototypes previously computed with another pre-trained CNN-model. Thus, as future work, we intend to modify the methodology to update the prototypes while the model learning cyclically. 
%At last, We also require to evaluate our PS-Layer in more challenging models and large databases. 


